Web Test Dependency Detection

E2E web test suites are prone to test dependencies due to the heterogeneous multi-tiered nature of modern web apps, which makes it difficult for developers to create isolated program states for each test case. In this paper, we present the first approach for detecting and validating test dependencies present in E2E web test suites. Our approach employs string analysis to extract an approximated set of dependencies from the test code. It then filters potential false dependencies through natural language processing of test names. Finally, it validates all dependencies, and uses a novel recovery algorithm to ensure no true dependencies are missed in the final test dependency graph. Our approach is implemented in a tool called TEDD and evaluated on the test suites of six open-source web apps. Our results show that TEDD can correctly detect and validate test dependencies up to 72% faster than the baseline with the original test ordering in which the graph contains all possible dependencies. The test dependency graphs produced by TEDD enable test execution parallelization, with a speed-up factor of up to 7x.

==> dependent-tests.tex <==
\def\tikzmark#1{\tikz[remember picture,overlay]\node[yshift=2pt](#1){};}

\begin{figure}[t]
\centering

\begin{lstlisting}[]
@Test
public void addUserTest() {
	driver.findElement(By.id("login")).sendKeys(<@\hlsmooth{"admin"}@>);
	driver.findElement(By.id("password")).sendKeys(<@\hlsmooth{"admin"}@>);
	driver.findElement(By.xpath("//button")).click();
	driver.findElement(By.linkText("Platform administration")).click();
	driver.findElement(By.linkText("Create user")).click();
	driver.findElement(By.id("lastname")).sendKeys(<@\hlsmooth{"Name001"}\tikzmark{A}@>);
	driver.findElement(By.id("firstname")).sendKeys(<@\hlsmooth{"Firstname001"}\tikzmark{B}@>); 
	driver.findElement(By.id("username")).sendKeys(<@\hlsmooth{"user001"}\tikzmark{C}@>);
	driver.findElement(By.id("password")).sendKeys(<@\hlsmooth{"password001"}@>);
	driver.findElement(By.id("password_conf")).sendKeys(<@\hlsmooth{"password001"}@>);
	assertEquals("The new user has been created", driver.findElement(By.xpath("//*[@id='claroBody']")).getText());
	driver.findElement(By.id("logout")).click();
}
@Test
public void searchUserTest() {
	driver.findElement(By.id("login")).sendKeys(<@\hlsmooth{"admin"}@>);
	driver.findElement(By.id("password")).sendKeys(<@\hlsmooth{"admin"}@>);
	driver.findElement(By.xpath("//button")).click();
	driver.findElement(By.linkText("Platform administration")).click();
	driver.findElement(By.id("search_user")).sendKeys(<@\hlsmooth{"user001"}\tikzmark{F}@>);
	driver.findElement(By.cssSelector("input[type='submit']")).click();
	assertEquals(<@\hlsmooth{"Name001"} \tikzmark{D}@>,driver.findElement(By.id("L0")).getText());
	assertEquals(<@\hlsmooth{"Firstname001"}\tikzmark{E}@>,driver.findElement(By.xpath("//td[3]")).getText());
	driver.findElement(By.id("logout")).click();
}
\end{lstlisting}

\tikzset{Empharrow/.style={gray,thick,dotted,->,arrows={Bar-Triangle[width=3pt]}}}

\begin{tikzpicture}[remember picture,overlay]
\draw[Empharrow](A)--+(0cm,0)--(D);
\draw[Empharrow](B)--+(0cm,0)--(E);
\draw[Empharrow](C)--+(0cm,0)--(F);
\end{tikzpicture}

\caption{\emph{Dependent E2E Selenium WebDriver web tests.}}
\label{fig:ab1} 
\end{figure}


==> graph.tex <==
\begin{figure}[h!]
\centering

\fbox{
%\includegraphics[trim=0.3cm 0cm 0.3cm 0cm, clip=true, scale=0.335]
%{images/dep-graph-string-claroline-BW-friendly.pdf}
\includegraphics[trim=0cm 20cm 0cm 0cm, clip=true, scale=0.11]
{images/graph.pdf}
}

\caption{\emph{Test dependency graph.}}
\label{fig:ab2}
\end{figure}


==> motivation-example.tex <==
\def\tikzmark#1{\tikz[remember picture,overlay]\node[yshift=2pt](#1){};}

\begin{figure*}[t]
\centering
\begin{subfigure}{\columnwidth}
\centering

\begin{lstlisting}[]
@Test
public void addUserTest() {
	driver.findElement(By.id("login")).sendKeys(<@\hlsmooth{"admin"}@>);
	driver.findElement(By.id("password")).sendKeys(<@\hlsmooth{"admin"}@>);
	driver.findElement(By.xpath("//button")).click();
	driver.findElement(By.linkText("Platform administration")).click();
	driver.findElement(By.linkText("Create user")).click();
	driver.findElement(By.id("lastname")).sendKeys(<@\hlsmooth{"Name001"}\tikzmark{A}@>);
	driver.findElement(By.id("firstname")).sendKeys(<@\hlsmooth{"Firstname001"}\tikzmark{B}@>); 
	driver.findElement(By.id("username")).sendKeys(<@\hlsmooth{"user001"}\tikzmark{C}@>);
	driver.findElement(By.id("password")).sendKeys(<@\hlsmooth{"password001"}@>);
	driver.findElement(By.id("password_conf")).sendKeys(<@\hlsmooth{"password001"}@>);
	assertEquals("The new user has been created", driver.findElement(By.xpath("//*[@id='claroBody']")).getText());
	driver.findElement(By.id("logout")).click();
}
@Test
public void searchUserTest() {
	driver.findElement(By.id("login")).sendKeys(<@\hlsmooth{"admin"}@>);
	driver.findElement(By.id("password")).sendKeys(<@\hlsmooth{"admin"}@>);
	driver.findElement(By.xpath("//button")).click();
	driver.findElement(By.linkText("Platform administration")).click();
	driver.findElement(By.id("search_user")).sendKeys(<@\hlsmooth{"user001"}\tikzmark{F}@>);
	driver.findElement(By.cssSelector("input[type='submit']")).click();
	assertEquals(<@\hlsmooth{"Name001"} \tikzmark{D}@>,driver.findElement(By.id("L0")).getText());
	assertEquals(<@\hlsmooth{"Firstname001"}\tikzmark{E}@>,driver.findElement(By.xpath("//td[3]")).getText());
	driver.findElement(By.id("logout")).click();
}
\end{lstlisting}

\tikzset{Empharrow/.style={gray,thick,dotted,->,arrows={Bar-Triangle[width=3pt]}}}

\begin{tikzpicture}[remember picture,overlay]
\draw[Empharrow](A)--+(0cm,0)--(D);
\draw[Empharrow](B)--+(0cm,0)--(E);
\draw[Empharrow](C)--+(0cm,0)--(F);
\end{tikzpicture}

\caption{\emph{Dependent E2E web tests.}}
\label{fig:ab1} 
\end{subfigure}
\qquad
\begin{subfigure}{\columnwidth}
\centering

%\fbox{
\includegraphics[trim=0.3cm 0cm 0.3cm 0cm, clip=true, scale=0.335]
{images/dep-graph-string-claroline-BW-friendly.pdf}
%}

\caption{\emph{Test dependency graph.}}
\label{fig:ab2}
\end{subfigure}
\caption{Two dependent E2E web tests for the Claroline web application from~\cite{WCRE}. \praw dependencies retrieved using input data string-based analysis are highlighted (\ref{fig:ab1}).
The test dependency graph for the test suite of our motivating example is shown in \ref{fig:ab2}. %, retrieved using input data string-based analysis.
Bold blue edges represent \textit{manifest} dependencies, namely dependencies that result in a different test result if they are not respected. 
Dashed red edges represent \textit{false} dependencies, while there are no \textit{missing} dependencies. %\textit{False} and \textit{manifest} dependencies are the result of the dynamic-analysis applied to the initial test dependency graph (see \autoref{sec:approach-da}).
} 
\label{fig:example} 
\end{figure*}


==> table-RQ1.tex <==
\begin{table*}[t]
\caption{RQ1}
\label{table-RQ1}
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1}

%\begin{tabular}{l@{\hskip 1.8em}llllll@{\hskip 1.8em}llllll@{\hskip 1.8em}llllll@{\hskip 1.8em}llllll@{\hskip 1.8em}llllll@{\hskip 1.8em}llllll}

\begin{tabular}{l@{\hskip 1em}lllll@{\hskip 1.8em}lllll@{\hskip 1.8em}lllll@{\hskip 1.8em}lllll@{\hskip 1.8em}lllll@{\hskip 1.8em}lllll@{\hskip 1.8em}lllll}

\toprule

& \multicolumn{5}{c}{\sc Claroline} 
& \multicolumn{5}{c}{\sc Addressbook}                                                                           & \multicolumn{5}{c}{\sc PPMA}                                                                                  & \multicolumn{5}{c}{\sc Collabtive}                                                                            & \multicolumn{5}{c}{\sc MRBS}                                                                                  & \multicolumn{5}{c}{\sc MantisBT}                                                                              & \multicolumn{5}{c}{All Apps} \\

\cmidrule(r){2-6} 
\cmidrule(r){7-11}
\cmidrule(r){12-16} 
\cmidrule(r){17-21}
\cmidrule(r){22-26} 
\cmidrule(r){27-31}
\cmidrule(r){32-36}

& \rot{Extracted}
& \rot{Filtered}
& \rot{False}
& \rot{Recovered}
& \rot{Manifest}

& \rot{Extracted}
& \rot{Filtered}
%& \multicolumn{3}{c}{\rot{Validation \& recovery}}
& \rot{False}

& \rot{Recovered}
& \rot{Manifest}

& \rot{Extracted}
& \rot{Filtered}
%& \multicolumn{3}{c}{\rot{Validation \& recovery}}
& \rot{False}

& \rot{Recovered}
& \rot{Manifest}

& \rot{Extracted}
& \rot{Filtered}
%& \multicolumn{3}{c}{\rot{Validation \& recovery}}
& \rot{False}

& \rot{Recovered}& \rot{Manifest}

& \rot{Extracted}
& \rot{Filtered}
%& \multicolumn{3}{c}{\rot{Validation \& recovery}}
& \rot{False}

& \rot{Recovered}& \rot{Manifest}

& \rot{Extracted}
& \rot{Filtered}
%& \multicolumn{3}{c}{\rot{Validation \& recovery}}
& \rot{False}

& \rot{Recovered}
& \rot{Manifest} 

& \rot{Extracted}
& \rot{Filtered}
%& \multicolumn{3}{c}{\rot{Validation \& recovery}}
& \rot{False}

& \rot{Recovered}
& \rot{Manifest} \\

\midrule

Complete & 780 & 780 & 738 & 0 & 42 & 351 & 351 & 320 & 0 & 31 & 253 & 253 & 231 & 0 & 22 & 780 & 780 & 740 & 0 & 40 & 231 & 231 & 210 & 0 & 21 & 820 & 820 & 785 & 0 & 35 & 536 & 536 & 504 & 0 & 32 \\
String Analysis & 601 & 601 & 559 & 2 & 42 & 351 & 67 & 36 & 9 & 31 & 253 & 56 & 36 & 8 & 20 & 746 & 107 & 65 & 25 & 42 & 231 & 87 & 66 & 4 & 21 & 784 & 96 & 60 & 16 & 36 & 494 & 169 & 137 & 11 & 32 \\ [0.5em]
NLP-Verb (Complete) & 780 & 561 & 519 & 0 & 42 & 351 & 187 & 156 & 0 & 31 & 253 & 91 & 69 & 0 & 22 & 780 & 702 & 662 & 0 & 40 & 231 & 160 & 139 & 0 & 21 & 820 & 796 & 761 & 0 & 35 & 536 & 416 & 384 & 0 & 32 \\
NLP-Verb (String Analysis) & 601 & 419 & 377 & 2 & 42 & 351 & 187 & 156 & 0 & 31 & 253 & 91 & 69 & 0 & 22 & 746 & 667 & 627 & 0 & 40 & 231 & 160 & 139 & 0 & 21 & 784 & 760 & 725 & 0 & 35 & 494 & 381 & 349 & 0 & 32 \\ [0.5em]
NLP-Dobj (Complete) & 780 & 210 & 168 & 13 & 42 & 351 & 131 & 99 & 0 & 32 & 253 & 51 & 29 & 5 & 22 & 780 & 185 & 144 & 8 & 41 & 231 & 90 & 67 & 5 & 23 & 820 & 378 & 340 & 7 & 38 & 536 & 174 & 141 & 6 & 33 \\
NLP-Dobj (String Analysis) & 601 & 144 & 101 & 15 & 43 & 351 & 131 & 99 & 0 & 32 & 253 & 51 & 29 & 5 & 22 & 746 & 150 & 108 & 9 & 42 & 231 & 90 & 67 & 5 & 23 & 784 & 342 & 304 & 7 & 38 & 494 & 151 & 118 & 7 & 33 \\ [0.5em]
NLP-Noun (Complete) & 780 & 325 & 285 & 5 & 40 & 351 & 85 & 54 & 4 & 31 & 253 & 46 & 24 & 6 & 22 & 780 & 189 & 149 & 4 & 40 & 231 & 84 & 59 & 3 & 25 & 820 & 300 & 265 & 2 & 35 & 536 & 172 & 139 & 4 & 32 \\
NLP-Noun (String Analysis) & 601 & 222 & 182 & 6 & 40 & 351 & 85 & 54 & 4 & 31 & 253 & 46 & 24 & 6 & 22 & 746 & 154 & 114 & 5 & 40 & 231 & 84 & 59 & 3 & 25 & 784 & 264 & 229 & 2 & 35 & 494 & 143 & 110 & 5 & 32 \\

\bottomrule
\end{tabular}
\end{table*}


==> table-RQ2-all.tex <==
\begin{table}[t]
\caption{RQ2}
\label{table:RQ2-runtime}
%\scriptsize
\setlength{\tabcolsep}{4.8pt}
\renewcommand{\arraystretch}{1}

%\begin{tabular}{l@{\hskip 0em}lllll@{\hskip 0em}llllll@{\hskip 0em}llllll@{\hskip 0em}llllll@{\hskip 0em}llllll@{\hskip 0em}llllll@{\hskip 0em}llllll@{\hskip 0em}llllll}
\begin{tabular}{lllllll}

\toprule

& \rot{Extraction} & \rot{Filtering} & \rot{Validation} & \rot{Recovery} & \rot{Total} & \rot{Saving (\%)} \\
 
\midrule
 
Complete & 0.00 & - & 425 & - & 425 & - \\
String Analysis & 0.10 & 0.00 & 195 & 5 & 200 & 53 \\ [0.5em]
NLP-Verb (Complete) & 0.00 & 0.04 & 307 & 1 & 309 & 27 \\
NLP-Verb (String Analysis) & 0.09 & 0.04 & 281 & 1 & 283 & 33 \\[0.5em]
NLP-Dobj (Complete) & 0.00 & 0.24 & 135 & 3 & 139 & 67 \\
NLP-Dobj (String Analysis) & 0.09 & 0.23 & 129 & 9 & 139 & 67 \\[0.5em]
NLP-Noun (Complete) & 0.00 & 0.05 & 123 & 3 & 126 & 70 \\
NLP-Noun (String Analysis) & 0.08 & 0.04 & 116 & 4 & 120 & 72 \\

\bottomrule

\end{tabular}
\end{table}



==> table-RQ2-nofit.tex <==
\begin{table*}[t]
\scriptsize
\setlength{\tabcolsep}{2pt}

\begin{tabular}{lllllllllllllllllllllllllllllllllllllllllllllllllllllll}

\toprule

& \multicolumn{5}{c}{\sc Complete} &
\multicolumn{5}{c}{\sc SA} &
\multicolumn{5}{c}{\sc NLP-VERB-C} &
\multicolumn{5}{c}{\sc NLP-VERB-SA} &
\multicolumn{5}{c}{\sc NLP-DOBJ-C} &
\multicolumn{5}{c}{\sc NLP-DOBJ-SA} &
\multicolumn{5}{c}{\sc NLP-NOUN-B} &
\multicolumn{5}{c}{\sc NLP-NOUN-SA} & \\

\cmidrule(r){2-6} \cmidrule(r){7-12}
\cmidrule(r){13-18} \cmidrule(r){20-25}
\cmidrule(r){26-31} \cmidrule(r){32-37} \\

 & \rot{Extraction}
 & \rot{Filtering}
 & \rot{Validation}
 & \rot{Recovery}
 & \rot{Total}
 & \rot{Extraction}
 & \rot{Filtering}
 & \rot{Validation}
 & \rot{Recovery}
 & \rot{Total}
 & \rot{Overhead (\%)}
 & \rot{Saving (\%)}
 & \rot{Extraction}
 & \rot{Filtering}
 & \rot{Validation}
 & \rot{Recovery}
 & \rot{Total}
 & \rot{Overhead (\%)}
 & \rot{Saving (\%)}
 & \rot{Extraction}
 & \rot{Filtering}
 & \rot{Validation}
 & \rot{Recovery}
 & \rot{Total}
 & \rot{Overhead (\%)}
 & \rot{Saving (\%)}
 & \rot{Extraction}
 & \rot{Filtering}
 & \rot{Validation}
 & \rot{Recovery}
 & \rot{Total}
 & \rot{Overhead (\%)}
 & \rot{Saving (\%)}
 & \rot{Extraction}
 & \rot{Filtering}
 & \rot{Validation}
 & \rot{Recovery}
 & \rot{Total}
 & \rot{Overhead (\%)}
 & \rot{Saving (\%)}
 & \rot{Extraction}
 & \rot{Filtering}
 & \rot{Validation}
 & \rot{Recovery}
 & \rot{Total}
 & \rot{Overhead (\%)}
 & \rot{Saving (\%)}
 & \rot{Extraction}
 & \rot{Filtering}
 & \rot{Validation}
 & \rot{Recovery}
 & \rot{Total}
 & \rot{Overhead (\%)}
 & \rot{Saving (\%)} \\

\midrule

Claroline   & 0        & 0    & 614   & 0    & 614   & 0.10 & 0    & 305.4  & 1.8   & 307   & 0.03\%        & 50\%        & 0          & 0.05 & 229   & 2    & 230   & 0.02\%        & 62\%        & 0.10        & 0.04 & 184   & 2    & 186   & 0.08\%        & 70\%        & 0          & 0.3   & 132  & 2     & 134   & 0.20\%        & 78\%        & 0.10        & 0.2   & 97   & 16    & 113   & 0.3\%         & 82\%        & 0          & 0.06 & 147  & 2    & 149   & 0.04\%        & 76\%        & 0.10        & 0.04 & 104  & 11    & 115   & 0.12\%        & 81\%        \\
Addressbook & 0        & 0    & 88    & 0    & 88    & 0.09 & 0    & 51.6   & 1.3   & 53    & 0.18\%        & 40\%        & 0          & 0.04 & 34    & 1    & 35    & 0.11\%        & 60\%        & 0.07        & 0.03 & 34    & 1    & 35    & 0.29\%        & 60\%        & 0          & 0.2   & 27   & 1     & 28    & 0.80\%        & 68\%        & 0.08        & 0.2   & 27   & 1     & 28    & 1.0\%         & 68\%        & 0          & 0.04 & 26   & 6    & 32    & 0.13\%        & 64\%        & 0.08        & 0.04 & 26   & 6     & 32    & 0.35\%        & 63\%        \\
PPMA        & 0        & 0    & 80    & 0    & 80    & 0.08 & 0    & 36.0   & 17.1  & 53    & 0.15\%        & 33\%        & 0          & 0.04 & 18    & 0    & 18    & 0.20\%        & 77\%        & 0.07        & 0.03 & 18    & 0    & 18    & 0.55\%        & 77\%        & 0          & 0.2   & 31   & 2     & 33    & 0.63\%        & 58\%        & 0.06        & 0.2   & 31   & 2     & 33    & 0.8\%         & 58\%        & 0          & 0.04 & 31   & 2    & 32    & 0.13\%        & 60\%        & 0.06        & 0.04 & 31   & 2     & 32    & 0.30\%        & 60\%        \\
Collabtive  & 0        & 0    & 1215  & 0    & 1215  & 0.12 & 0    & 543.0  & 3.1   & 546   & 0.02\%        & 55\%        & 0          & 0.04 & 1066  & 2    & 1068  & 0.00\%        & 12\%        & 0.10        & 0.04 & 959   & 2    & 962   & 0.01\%        & 21\%        & 0          & 0.3   & 342  & 2     & 344   & 0.08\%        & 72\%        & 0.10        & 0.3   & 355  & 22    & 377   & 0.1\%         & 69\%        & 0          & 0.05 & 275  & 2    & 278   & 0.02\%        & 77\%        & 0.10        & 0.04 & 288  & 2     & 290   & 0.05\%        & 76\%        \\
MRBS        & 0        & 0    & 79    & 0    & 79    & 0.08 & 0    & 36.0   & 1.3   & 37    & 0.23\%        & 52\%        & 0          & 0.04 & 45    & 0    & 45    & 0.10\%        & 43\%        & 0.07        & 0.03 & 45    & 0    & 45    & 0.21\%        & 42\%        & 0          & 0.2   & 33   & 12    & 45    & 0.50\%        & 43\%        & 0.07        & 0.2   & 33   & 12    & 45    & 0.6\%         & 43\%        & 0          & 0.05 & 32   & 1    & 34    & 0.15\%        & 57\%        & 0.07        & 0.04 & 32   & 1     & 34    & 0.30\%        & 57\%        \\
MantisBT    & 0        & 0    & 472   & 0    & 472   & 0.11 & 0    & 198.6  & 3.6   & 202   & 0.06\%        & 57\%        & 0          & 0.05 & 452   & 3    & 454   & 0.01\%        & 4\%         & 0.10        & 0.05 & 446   & 3    & 449   & 0.03\%        & 5\%         & 0          & 0.3   & 244  & 2     & 247   & 0.11\%        & 48\%        & 0.10        & 0.3   & 233  & 2     & 235   & 0.2\%         & 50\%        & 0          & 0.07 & 229  & 2    & 231   & 0.03\%        & 51\%        & 0.10        & 0.06 & 216  & 2     & 219   & 0.07\%        & 54\%        \\


 \bottomrule
 \end{tabular}
 \label{table:RQ2}
\end{table*}


==> table-RQ2-runtime.tex <==
\begin{table*}[t]
\caption{RQ2}
\label{table:RQ2-runtime}
\scriptsize
\setlength{\tabcolsep}{1.4pt}
\renewcommand{\arraystretch}{1}

\begin{tabular}{l@{\hskip 0em}lllll@{\hskip 0em}llllll@{\hskip 0em}llllll@{\hskip 0em}llllll@{\hskip 0em}llllll@{\hskip 0em}llllll@{\hskip 0em}llllll@{\hskip 0em}llllll}

\toprule

& \multicolumn{5}{c}{\sc Complete} &
\multicolumn{6}{c}{\sc SA} &
\multicolumn{6}{c}{\sc NLP-VERB-C} &
\multicolumn{6}{c}{\sc NLP-VERB-SA} &
\multicolumn{6}{c}{\sc NLP-DOBJ-C} &
\multicolumn{6}{c}{\sc NLP-DOBJ-SA} &
\multicolumn{6}{c}{\sc NLP-NOUN-B} &
\multicolumn{6}{c}{\sc NLP-NOUN-SA} \\

\cmidrule(r){2-6} \cmidrule(r){7-12}
\cmidrule(r){13-18} \cmidrule(r){19-24}
\cmidrule(r){25-30} \cmidrule(r){31-36}
\cmidrule(r){37-42} \cmidrule(r){43-48}

& \rot{Extraction} & \rot{Filtering} & \rot{Validation} & \rot{Recovery} & \rot{Total}
& \rot{Extraction} & \rot{Filtering} & \rot{Validation} & \rot{Recovery} & \rot{Total} & \rot{Saving (\%)}
& \rot{Extraction} & \rot{Filtering} & \rot{Validation} & \rot{Recovery} & \rot{Total} & \rot{Saving (\%)}
& \rot{Extraction} & \rot{Filtering} & \rot{Validation} & \rot{Recovery} & \rot{Total} & \rot{Saving (\%)}
& \rot{Extraction} & \rot{Filtering} & \rot{Validation} & \rot{Recovery} & \rot{Total} & \rot{Saving (\%)}
& \rot{Extraction} & \rot{Filtering} & \rot{Validation} & \rot{Recovery} & \rot{Total} & \rot{Saving (\%)}
& \rot{Extraction} & \rot{Filtering} & \rot{Validation} & \rot{Recovery} & \rot{Total} & \rot{Saving (\%)}
& \rot{Extraction} & \rot{Filtering} & \rot{Validation} & \rot{Recovery} & \rot{Total} & \rot{Saving (\%)}  \\

\midrule

Claroline & 0 & 0 & 614 & 0 & 614 & 0.10 & 0 & 305.4 & 1.8 & 307 & 50 & 0 & 0.05 & 229 & 2 & 230 & 62 & 0.10 & 0.04 & 184 & 2 & 186 & 70 & 0 & 0.3 & 132 & 2 & 134 & 78 & 0.10 & 0.2 & 97 & 16 & 113 & 82 & 0 & 0.06 & 147 & 2 & 149 & 76 & 0.10 & 0.04 & 104 & 11 & 115 & 81 \\

Addressbook & 0 & 0 & 88 & 0 & 88 & 0.09 & 0 & 51.6 & 1.3 & 53 & 40 & 0 & 0.04 & 34 & 1 & 35 & 60 & 0.07 & 0.03 & 34 & 1 & 35 & 60 & 0 & 0.2 & 27 & 1 & 28 & 68 & 0.08 & 0.2 & 27 & 1 & 28 & 68 & 0 & 0.04 & 26 & 6 & 32 & 64 & 0.08 & 0.04 & 26 & 6 & 32 & 63 \\

PPMA & 0 & 0 & 80 & 0 & 80 & 0.08 & 0 & 36.0 & 17.1 & 53 & 33 & 0 & 0.04 & 18 & 0 & 18 & 77 & 0.07 & 0.03 & 18 & 0 & 18 & 77 & 0 & 0.2 & 31 & 2 & 33 & 58 & 0.06 & 0.2 & 31 & 2 & 33 & 58 & 0 & 0.04 & 31 & 2 & 32 & 60 & 0.06 & 0.04 & 31 & 2 & 32 & 60 \\

Collabtive & 0 & 0 & 1215 & 0 & 1215 & 0.12 & 0 & 543.0 & 3.1 & 546 & 55 & 0 & 0.04 & 1066 & 2 & 1068 & 12 & 0.10 & 0.04 & 959 & 2 & 962 & 21 & 0 & 0.3 & 342 & 2 & 344 & 72 & 0.10 & 0.3 & 355 & 22 & 377 & 69 & 0 & 0.05 & 275 & 2 & 278 & 77 & 0.10 & 0.04 & 288 & 2 & 290 & 76 \\

MRBS & 0 & 0 & 79 & 0 & 79 & 0.08 & 0 & 36.0 & 1.3 & 37 & 52 & 0 & 0.04 & 45 & 0 & 45 & 43 & 0.07 & 0.03 & 45 & 0 & 45 & 42 & 0 & 0.2 & 33 & 12 & 45 & 43 & 0.07 & 0.2 & 33 & 12 & 45 & 43 & 0 & 0.05 & 32 & 1 & 34 & 57 & 0.07 & 0.04 & 32 & 1 & 34 & 57 \\

MantisBT & 0 & 0 & 472 & 0 & 472 & 0.11 & 0 & 198.6 & 3.6 & 202 & 57 & 0 & 0.05 & 452 & 3 & 454 & 4 & 0.10 & 0.05 & 446 & 3 & 449 & 5 & 0 & 0.3 & 244 & 2 & 247 & 48 & 0.10 & 0.3 & 233 & 2 & 235 & 50 & 0 & 0.07 & 229 & 2 & 231 & 51 & 0.10 & 0.06 & 216 & 2 & 219 & 54 \\

\midrule

Average & 0 & 0 & 425 & 0 & 425 & 0.10 & 0 & 195.1 & 4.7 & 200 & \textbf{48} & 0 & 0.04 & 307 & 1 & 309 & \textbf{43} & 0.09 & 0.04 & 281 & 1 & 283 & \textbf{46} & 0 & 0.2 & 135 & 3 & 139 & \textbf{61} & 0.09 & 0.2 & 129 & 9 & 139 & \textbf{62} & 0 & 0.05 & 123 & 3 & 126 & \textbf{64} & 0.08 & 0.04 & 116 & 4 & 120 & \textbf{65} \\


\bottomrule
\end{tabular}
\end{table*}


==> table-all-RQs.tex <==
\begin{table*}[]

\caption{RQs}
\label{table-RQs}
%\scriptsize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1}

\begin{tabular}{@{}l@{\hskip 2em}lllll@{\hskip 2em}llllll@{\hskip 2em}lll@{}}

\toprule 

& \multicolumn{5}{c}{\sc Effectiveness} 
& \multicolumn{6}{c}{\sc Performance} 
& \multicolumn{3}{c}{\sc Parallelization} \\

\cmidrule(r){2-6} 
\cmidrule(r){7-12}
\cmidrule(r){13-15}

& \rot{Extracted}
& \rot{Filtered}
& \rot{False}
& \rot{Recovered}
& \rot{Manifest}

& \rot{Extraction} 
& \rot{Filtering} 
& \rot{Validation} 
& \rot{Recovery} 
& \rot{Total}
& \rot{Saving (\%)}

& \rot{Unique schedules} 
& \rot{Speedup (worst)} 
& \rot{Speedup (average)} \\

\midrule 

Complete & 536 & 536 & 504 & 0 & 32 & 0.00 & - & 425 & - & 425 & - & 30 & 2.2$\times$ & 7.1 \\
String Analysis & 494 & 169 & 137 & 11 & 32 & 0.10 & 0.00 & 195 & 5 & 200 & 53\% & 30 & 2.3 & 7.2 \\ [0.5em]
NLP-Verb (Complete) & 536 & 416 & 384 & 0 & 32 & 0.00 & 0.04 & 307 & 1 & 309 & 27\% & 30 & 2.2 & 7.1 \\
NLP-Verb (String Analysis) & 494 & 381 & 349 & 0 & 32 & 0.09 & 0.04 & 281 & 1 & 283 & 33\% & 30 & 2.2 & 7.1 \\ [0.5em]
NLP-Dobj (Complete) & 536 & 174 & 141 & 6 & 33 & 0.00 & 0.24 & 135 & 3 & 139 & 67\% & 29 & 2.1 & 6.7 \\
NLP-Dobj (String Analysis) & 494 & 151 & 118 & 7 & 33 & 0.09 & 0.23 & 129 & 9 & 139 & 67\% & 29 & 2.1 & 6.7 \\ [0.5em]
NLP-Noun (Complete) & 536 & 172 & 139 & 4 & 32 & 0.00 & 0.05 & 123 & 3 & 126 & 70\% & 29 & 2.1 & 6.7 \\
NLP-Noun (String Analysis) & 494 & 143 & 110 & 5 & 32 & 0.08 & 0.04 & 116 & 4 & 120 & 72\% & 29 & 2.1 & 6.8 \\

\bottomrule

\end{tabular}

\end{table*}

